QPruner: Probabilistic Decision Quantization for Structured Pruning in Large Language Models

The rise of large language models (LLMs) has significantly advanced various natural language processing (NLP) tasks. However, the resource demands of these models pose substantial challenges. Structured pruning is an effective approach to reducing model size, but it often results in significant accuracy degradation, necessitating parameter updates to adapt. Unfortunately, such fine-tuning requires substantial memory, which limits its applicability. To address these challenges, we introduce quantization into the structured pruning framework to reduce memory consumption during both fine-tuning and inference. However, the combined errors from pruning and quantization increase the difficulty of fine-tuning, requiring a more refined quantization scheme. To this end, we propose QPruner, a novel framework that employs structured pruning to reduce model size, followed by a layer-wise mixed-precision quantization scheme. Quantization precisions are assigned to each layer based on their importance to the target task, and Bayesian optimization is employed to refine precision allocation strategies, ensuring a balance between model accuracy and memory efficiency. Extensive experiments on benchmark datasets demonstrate that QPruner significantly outperforms existing methods in memory savings while maintaining or improving model performance.

==> tabs/tab__ablation.tex <==
\begin{table*}[ht]
\centering
\caption{Performance comparison for the ablation study under the overall best $R$ configuration for seven tasks on LLaMA-7B. The results are reported in percentage (\%).}
\label{tab:Ablation}
\resizebox{\linewidth}{!}
{
\begin{tabular}{lcc|cc|ccc|ccc}
\toprule
\multirow{2}{*}{Benchmark} & \multicolumn{2}{c}{Sample Size} & \multicolumn{2}{c}{Element-wise Importance} & \multicolumn{3}{c}{Setting of Performance Model} & \multicolumn{3}{c}{Micro-batch Size} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
 & $N$=10 & $N$=50 &  Element\textsuperscript{1} & Element\textsuperscript{2} & Setting1 & Setting2 & Setting3 & Micro-4 & Micro-8 & Micro-16 \\
\midrule
ARC-e       & 63.97 & \textbf{65.32} & \textbf{63.97} & 62.84 & 63.97 & 64.73 & 64.65 & 64.52 & 63.97 & \textbf{65.24} \\
ARC-c       & 37.29 & \textbf{37.71} & \textbf{37.29} & 36.77 & 37.29 & 36.60 & \textbf{37.54} & \textbf{38.65} & 37.29 & 37.54 \\
WinoGrande  & \textbf{63.61} & 63.14 & \textbf{63.61} & 63.22 & 63.61 & \textbf{63.46} & 63.06 & 62.04 & \textbf{63.61} & 63.14 \\
OBQA        & \textbf{39.80} & \textbf{41.00} & \textbf{39.80} & 39.80 & 39.80 & \textbf{40.80} & \textbf{40.80} & 40.00 & 39.80 & \textbf{40.80} \\
BoolQ       & \textbf{65.81} & 64.43 & 65.81 & \textbf{66.48} & \textbf{66.91} & 64.43 & 64.86 & \textbf{67.28} & 65.81 & 66.91 \\
PIQA        & 76.99 & \textbf{77.15} & \textbf{76.99} & 76.82 & 76.99 & 76.99 & \textbf{77.04} & 76.50 & \textbf{76.99} & 76.93 \\
HellaSwag   & \textbf{68.56} & 68.52 & \textbf{68.56} & 67.88 & 68.56 & 68.75 & \textbf{69.00} & 68.08 & 68.56 & \textbf{68.78} \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tabs/tab__con-llama13b.tex <==
\begin{table*}[ht]
    \centering
    \caption{Specific Composition of $R$ in LLaMA-7B Experiment}
    \resizebox{\linewidth}{!}
    {
        \begin{tabular}{cc|c}
            \toprule
             Pruning Rate &Tasks& Layers' Rank Values (1\textasciitilde 32/40) \\
            \midrule
              \multirow{7}{*}{20\%} & BoolQ & 8, 8, 8, 8, 4, 12, 12, 12, 12, 10, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 10, 6, 4, 4, 4, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &PIQA&8, 8, 8, 8, 4, 12, 12, 12, 12, 10, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 10, 6, 4, 4, 4, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &Hella&8, 8, 8, 8, 2, 2, 4, 10, 10, 6, 10, 10, 10, 6, 6, 2, 2, 10, 2, 4, 2, 10, 10, 10, 4, 10, 10, 6, 6, 2, 8, 8\\
             \cmidrule{2-3}
             &Wino&8, 8, 8, 8, 8, 10, 4, 10, 4, 6, 6, 2, 10, 8, 12, 12, 10, 12, 12, 10, 6, 6, 8, 8, 10, 6, 6, 12, 2, 8, 8, 8\\
             \cmidrule{2-3}
             &ARC-e&8, 8, 8, 8, 4, 12, 12, 12, 12, 10, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 10, 6, 4, 4, 4, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &ARC-c&8, 8, 8, 8, 4, 12, 12, 12, 12, 10, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 10, 6, 4, 4, 4, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &OBQA&8, 8, 8, 8, 4, 12, 12, 12, 12, 10, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 10, 6, 4, 4, 4, 2, 12, 8, 8\\
            \cmidrule{1-3}
             \multirow{7}{*}{25\%} & BoolQ & 8, 8, 8, 8, 12, 2, 8, 2, 8, 12, 4, 2, 10, 12, 10, 4, 2, 2, 12, 8, 10, 2, 12, 12, 8, 4, 4, 2, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &PIQA&8, 8, 8, 8, 4, 2, 2, 10, 10, 2, 10, 10, 10, 2, 2, 2, 4, 10, 4, 6, 10, 2, 2, 6, 10, 2, 2, 10, 10, 2, 8, 8\\
             \cmidrule{2-3}
             &Hella&8, 8, 8, 8, 4, 10, 12, 12, 6, 10, 6, 6, 8, 2, 2, 12, 2, 12, 12, 6, 4, 10, 6, 2, 2, 8, 4, 2, 2, 8, 8, 8\\
             \cmidrule{2-3}
             &Wino&8, 8, 8, 8, 8, 4, 12, 8, 2, 2, 12, 2, 10, 12, 2, 12, 12, 10, 8, 12, 4, 6, 6, 4, 10, 4, 2, 10, 10, 12, 8, 8\\
             \cmidrule{2-3}
             &ARC-e&8, 8, 8, 8, 2, 12, 2, 6, 12, 6, 12, 10, 6, 4, 8, 8, 12, 2, 2, 6, 8, 4, 12, 12, 2, 4, 2, 6, 6, 2, 8, 8\\
             \cmidrule{2-3}
             &ARC-c&8, 8, 8, 8, 2, 12, 2, 6, 12, 6, 12, 10, 6, 4, 8, 8, 12, 2, 2, 6, 8, 4, 12, 12, 2, 4, 2, 6, 6, 2, 8, 8\\
             \cmidrule{2-3}
             &OBQA&8, 8, 8, 8, 4, 12, 12, 12, 12, 1, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 12, 10, 4, 4, 6, 2, 12, 8, 8\\
            \cmidrule{1-3}
              \multirow{7}{*}{30\%} & BoolQ & 8, 8, 8, 8, 12, 2, 8, 2, 8, 12, 4, 2, 10, 12, 10, 4, 2, 2, 12, 8, 10, 2, 12, 12, 8, 4, 4, 2, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &PIQA&8, 8, 8, 8, 12, 6, 10, 4, 2, 4, 2, 4, 12, 8, 2, 2, 2, 12, 12, 12, 12, 2, 12, 4, 4, 2, 10, 2, 2, 8, 8, 8\\
             \cmidrule{2-3}
             &Hella&8, 8, 8, 8, 12, 6, 8, 4, 2, 12, 10, 4, 4, 2, 6, 4, 6, 10, 4, 2, 8, 6, 12, 10, 4, 6, 6, 6, 8, 2, 8, 8\\
             \cmidrule{2-3}
             &Wino&8, 8, 8, 8, 12, 6, 8, 4, 2, 12, 10, 4, 4, 2, 6, 4, 6, 10, 4, 2, 8, 6, 12, 10, 4, 6, 6, 6, 8, 2, 8, 8\\
             \cmidrule{2-3}
             &ARC-e&8, 8, 8, 8, 12, 6, 8, 4, 2, 12, 10, 4, 4, 2, 6, 4, 6, 10, 4, 2, 8, 6, 12, 10, 4, 6, 6, 6, 8, 2, 8, 8\\
             \cmidrule{2-3}
             &ARC-c&8, 8, 8, 8, 4, 10, 12, 12, 6, 10, 6, 6, 8, 2, 2, 12, 2, 12, 12, 6, 4, 10, 6, 2, 2, 8, 4, 2, 2, 8, 8, 8\\
             \cmidrule{2-3}
             &OBQA&8, 8, 8, 8, 12, 6, 8, 4, 2, 12, 10, 4, 4, 2, 6, 4, 6, 10, 4, 2, 8, 6, 12, 10, 4, 6, 6, 6, 8, 2, 8, 8\\
            \cmidrule{1-3}
             \multirow{7}{*}{50\%} & BoolQ & 8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &PIQA&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &Hella&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &Wino&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &ARC-e&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &ARC-c&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &OBQA&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
            \bottomrule
        \end{tabular}
    }\label{tab:con-llama13b}
\end{table*}

==> tabs/tab__main.tex <==
\begin{table*}[t]
    \centering
    \caption{Zero-shot performance of LLaMA-7B in unpruned, pruned, LoRA recovery, and RankAdaptor recovery. ‘Bold’ indicates the best performance at each pruning rate. Results are the optimal performance for each task. Specific $R$ configurations in Appendix \ref{app:r}. Reported in percentage (\%).}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{ll|ccccccc}
            \toprule
            Pruning Rate & Recover & BoolQ & PIQA & HellaSwag & WinoGrande & ARC-e & ARC-c & OBQA  \\
            \midrule
            {\parbox{1.8cm}{Rate = 0\%}} & - & 73.09 & 78.35 & 72.98 & 67.09 & 67.42 & 41.38 & 42.40  \\
            \cmidrule{1-9}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 20\%}} & w/o Tuning & 56.94 & 75.73 & 66.83 & 60.06 & 60.94 & 36.43 & 39.80 \\
            \cmidrule{2-9}
            & LoRA  & 63.30 & 76.82 & 68.68 & 63.38 & 63.76 & 37.11 & 40.60   \\
            \cmidrule{2-9}
            & RankAdaptor & \textbf{67.34} & \textbf{77.31} & \textbf{69.07} & \textbf{64.17} & \textbf{65.36} & \textbf{37.80} & \textbf{41.60}  \\
            \cmidrule{1-9}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 25\%}} & w/o Tuning & 59.94 & 73.23 & 62.35 & 58.80 & 55.81 & 34.90 & 39.40 \\
            \cmidrule{2-9}
            & LoRA  & 61.93 & 76.01 & 65.97 & 61.96 & 62.21 & 35.92 & 39.40  \\
            \cmidrule{2-9}
            & RankAdaptor & \textbf{67.43} & \textbf{76.06} & \textbf{66.08} & \textbf{64.40} & \textbf{62.63} & \textbf{36.77} & \textbf{40.40} \\
            \cmidrule{1-9}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 30\%}} & w/o Tuning & 58.96 & 71.22 & 58.10 & 58.88 & 52.19 & 32.34 & 38.40 \\
            \cmidrule{2-9}
            & LoRA  & 62.45 & 74.37 & 63.14 & 61.96 & 59.22 & 33.70 & 39.60  \\
            \cmidrule{2-9}
            & RankAdaptor & \textbf{66.21} & \textbf{75.19} & \textbf{63.61} & \textbf{63.14} & \textbf{60.10} & \textbf{34.64} & \textbf{40.20} \\
            \cmidrule{1-9}
            \multirow{5}{*}{\parbox{1.8cm}{Rate = 50\%}} & w/o Tuning & \textbf{57.98} & 60.94 & 34.35 & \textbf{52.25} & 31.82 & 27.30 & \textbf{35.80} \\
            \cmidrule{2-9}
            & LoRA  & 43.76 & 69.04 & 45.01 & 50.99 & 45.20 & \textbf{28.75} & 34.60   \\
            \cmidrule{2-9}
            & RankAdaptor & 51.65 & \textbf{69.48} & \textbf{45.03} & 51.93 & \textbf{45.66} & 28.41 & 35.00  \\
            \bottomrule
        \end{tabular}
    }\label{tab:res-llama7b}
\end{table*}

==> tabs/tab__mov.tex <==
\begin{table}
    \centering
    \begin{tabular}{c|c|c}
        \hline
        \text{Layer}  & \text{Fixed} & \text{Different} \\
        \hline
        1--8  & \multirow{4}{*}{8} & 4 \\
        9--16  &  & 6 \\
        17--24  &  & 10 \\
        25--32  &  & 12 \\
        \hline
    \end{tabular}
    \caption{Rank Value Configurations. Fixed refers to applying a constant rank value across multiple layers of the pruned model, while Different indicates assigning distinct rank values to different layers of the pruned model.}
    \label{tab:moti_config}
\end{table}

==> tabs/tab__res-llama13b.tex <==
\begin{table*}[ht]
    \centering
    \caption{Zero-shot performance of LLaMA-13B in unpruned, pruned, pruned with LoRA recovery, and pruned with RankAdaptor recovery settings; 'Bold' represents the best performance at the same pruning rate across the three pruned settings. The data in the table is from the optimal performance on each individual task. The results are reported in percentage (\%).}
    \resizebox{0.866\linewidth}{!}{
        \begin{tabular}{ll|ccccccc}
            \toprule
            Pruning Rate & Recover & BoolQ & PIQA & HellaSwag & WinoGrande & ARC-e & ARC-c & OBQA \\
            \midrule
            {\parbox{1.8cm}{Rate = 0\%}} & N/A & 68.50 & 79.11 & 76.21 & 70.09 & 74.58 & 44.54 & 42.20  \\
            \cmidrule{1-9}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 50\%}} & W/O Tuning & 58.90 & 66.32 & 42.24 & 52.25 & 39.06 & 29.18 & 33.20 \\
            \cmidrule{2-9}
            & LoRA  & 61.93 & 71.38 & \textbf{53.36} & 53.59 & 53.11 & 29.95 & 38.00  \\
            \cmidrule{2-9}
            & RankAdaptor & \textbf{62.05} & \textbf{71.71} & 53.33 & \textbf{54.22} & \textbf{53.20} & \textbf{30.89} & \textbf{39.40} \\
            \bottomrule
        \end{tabular}
    }\label{tab:res-llama13b}
\end{table*}

==> tabs/tab__res-llama7b-avg.tex <==
\begin{table*}[t]
    \centering
    \caption{Zero-shot performance of LLaMA-7B in unpruned, pruned, pruned with LoRA recovery, and pruned with RankAdaptor recovery settings; 'Bold' represents the best performance at the same pruning rate across the three pruned settings. The data in the table is from the overall performance across multiple tasks. The results are reported in percentage (\%).}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{ll|ccccccc|c}
            \toprule
            Pruning Rate & Recover & BoolQ & PIQA & HellaSwag & WinoGrande & ARC-e & ARC-c & OBQA & Average \\
            \midrule
            {\parbox{1.8cm}{Rate = 0\%}} & N/A & 73.09 & 78.35 & 72.98 & 67.09 & 67.42 & 41.38 & 42.40 & 63.10 \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 20\%}} & W/O Tuning & 56.94 & 75.73 & 66.83 & 60.06 & 60.94 & 36.43 & 39.80 & 56.96 \\
            \cmidrule{2-10}
            & LoRA  & 63.30 & 76.82 & 68.68 & 63.38 & 63.76 & 37.11 & 40.60 & 59.52  \\
            \cmidrule{2-10}
            & RankAdaptor & 66.91 & 76.93 & 68.78 & 63.14 & 65.24 & 37.54 & 40.80 & \textbf{59.90}  \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 25\%}} & W/O Tuning & 59.94 & 73.23 & 62.35 & 58.80 & 55.81 & 34.90 & 39.40 & 54.63 \\
            \cmidrule{2-10}
            & LoRA  & 61.93 & 76.01 & 65.97 & 61.96 & 62.21 & 35.92 & 39.40 & 57.63  \\
            \cmidrule{2-10}
            & RankAdaptor & 63.15 & 75.95 & 65.97 & 62.04 & 62.63 & 36.77 & 39.60 & \textbf{58.16} \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 30\%}} & W/O Tuning & 58.96 & 71.22 & 58.10 & 58.88 & 52.19 & 32.34 & 38.40 & 52.58 \\
            \cmidrule{2-10}
            & LoRA  & 62.45 & 74.37 & 63.14 & 61.96 & 59.22 & 33.70 & 39.60 & 56.63  \\
            \cmidrule{2-10}
            & RankAdaptor & 62.72 & 74.39 & 63.61 & 63.14 & 60.10 & 33.62 & 40.20 & \textbf{56.97} \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 50\%}} & W/O Tuning & 57.98 & 60.94 & 34.35 & 52.25 & 31.82 & 27.30 & 35.80 & 42.92 \\
            \cmidrule{2-10}
            & LoRA  & 43.76 & 69.04 & 45.01 & 50.99 & 45.20 & 28.75 & 34.60 & 45.62   \\
            \cmidrule{2-10}
            & RankAdaptor & 51.65 & 69.48 & 45.03 & 51.93 & 45.66 & 28.41 & 35.00 & \textbf{46.74}  \\
            \bottomrule
        \end{tabular}
    }\label{tab:res-llama7b-avg}
\end{table*}

==> tabs/tab__res-vicuna7b.tex <==
\begin{table*}[ht]
    \centering
    \caption{Zero-shot performance of Vicuna-7B in unpruned, pruned, pruned with LoRA recovery, and pruned with RankAdaptor recovery settings; 'Bold' represents the best performance at the same pruning rate across the three pruned settings. The data in the table is from the optimal performance on each individual task. The results are reported in percentage (\%).}
    \resizebox{0.866\linewidth}{!}{
        \begin{tabular}{ll|ccccccc}
            \toprule
            Pruning Rate & Recover & BoolQ & PIQA & HellaSwag & WinoGrande & ARC-e & ARC-c & OBQA  \\
            \midrule
            {\parbox{1.8cm}{Rate = 0\%}} & - & 75.69 & 77.75 & 71.06 & 67.80 & 69.07 & 40.78 & 42.20  \\
            \cmidrule{1-9}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 20\%}} & W/O Tuning & 52.35 & 76.17 & 64.79 & 59.59 & 65.99 & \textbf{38.14} & 40.00 \\
            \cmidrule{2-9}
            & LoRA  & 57.77 & \textbf{77.58} & 67.16 & 63.14 & 67.30 & 37.71 & 40.40   \\
            \cmidrule{2-9}
            & RankAdaptor & \textbf{61.19} & 77.15 & \textbf{67.32} & \textbf{63.85} & \textbf{67.68} & 38.05 & \textbf{41.20}  \\
            \cmidrule{1-9}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 25\%}} & W/O Tuning & 43.98 & 74.76 & 61.58 & 57.06 & 63.72 & \textbf{37.20} & 39.80 \\
            \cmidrule{2-9}
            & LoRA  & 50.34 & 75.24 & 64.10 & 61.33 & \textbf{63.93} & 35.67 & 40.60   \\
            \cmidrule{2-9}
            & RankAdaptor & \textbf{58.50} & \textbf{76.17} & \textbf{64.23} & \textbf{61.96} & 63.30 & 36.01 & \textbf{42.00}  \\
            \cmidrule{1-9}
             \multirow{3}{*}{\parbox{1.8cm}{Rate = 30\%}} & W/O Tuning & 43.12 & 73.45 & 55.64 & 57.22 & 58.96 & 34.30 & 37.80 \\
            \cmidrule{2-9}
            & LoRA  & \textbf{58.81} & 74.37 & 60.70 & \textbf{60.62} & 59.01 & 33.79 & 38.80   \\
            \cmidrule{2-9}
            & RankAdaptor & 57.58 & \textbf{75.57} & \textbf{61.63} & 60.22 & \textbf{60.94} & \textbf{34.81} & \textbf{39.00} \\
            \cmidrule{1-9}
             \multirow{3}{*}{\parbox{1.8cm}{Rate = 50\%}} & W/O Tuning & \textbf{62.29} & 60.28 & 33.91 & \textbf{54.54} & 35.14 & \textbf{28.16} & 33.80 \\
            \cmidrule{2-9}
            & LoRA  & 59.51 & 66.87 & 43.18 & 52.01 & 48.40 & 26.45 & 34.00  \\
            \cmidrule{2-9}
            & RankAdaptor & 59.91 & \textbf{67.46} & \textbf{43.50} & 52.41 & \textbf{48.70} & 27.65 & \textbf{35.80} \\
            \bottomrule
        \end{tabular}
    }\label{tab:res-vicuna7b}
\end{table*}

==> tabs/tab_ablation.tex <==
\begin{table*}[ht]
\centering
\caption{Performance comparison for the ablation study under the overall best $R$ configuration for seven tasks on LLaMA-7B. The results are reported in percentage (\%).}
\label{tab:Ablation}
\resizebox{\linewidth}{!}
{
\begin{tabular}{lcc|cc|ccc|ccc}
\toprule
\multirow{2}{*}{Benchmark} & \multicolumn{2}{c}{Sample Size} & \multicolumn{2}{c}{Element-wise Importance} & \multicolumn{3}{c}{Setting of Performance Model} & \multicolumn{3}{c}{Micro-batch Size} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
 & $N$=10 & $N$=50 &  Element\textsuperscript{1} & Element\textsuperscript{2} & Setting1 & Setting2 & Setting3 & Micro-4 & Micro-8 & Micro-16 \\
\midrule
ARC-e       & 63.97 & \textbf{65.32} & \textbf{63.97} & 62.84 & 63.97 & 64.73 & 64.65 & 64.52 & 63.97 & \textbf{65.24} \\
ARC-c       & 37.29 & \textbf{37.71} & \textbf{37.29} & 36.77 & 37.29 & 36.60 & \textbf{37.54} & \textbf{38.65} & 37.29 & 37.54 \\
WinoGrande  & \textbf{63.61} & 63.14 & \textbf{63.61} & 63.22 & 63.61 & \textbf{63.46} & 63.06 & 62.04 & \textbf{63.61} & 63.14 \\
OBQA        & \textbf{39.80} & \textbf{41.00} & \textbf{39.80} & 39.80 & 39.80 & \textbf{40.80} & \textbf{40.80} & 40.00 & 39.80 & \textbf{40.80} \\
BoolQ       & \textbf{65.81} & 64.43 & 65.81 & \textbf{66.48} & \textbf{66.91} & 64.43 & 64.86 & \textbf{67.28} & 65.81 & 66.91 \\
PIQA        & 76.99 & \textbf{77.15} & \textbf{76.99} & 76.82 & 76.99 & 76.99 & \textbf{77.04} & 76.50 & \textbf{76.99} & 76.93 \\
HellaSwag   & \textbf{68.56} & 68.52 & \textbf{68.56} & 67.88 & 68.56 & 68.75 & \textbf{69.00} & 68.08 & 68.56 & \textbf{68.78} \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tabs/tab_con-llama13b.tex <==
\begin{table*}[ht]
    \centering
    \caption{Specific Composition of $R$ in LLaMA-7B Experiment}
    \resizebox{\linewidth}{!}
    {
        \begin{tabular}{cc|c}
            \toprule
             Pruning Rate &Tasks& Layers' Rank Values (1\textasciitilde 32/40) \\
            \midrule
              \multirow{7}{*}{20\%} & BoolQ & 8, 8, 8, 8, 4, 12, 12, 12, 12, 10, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 10, 6, 4, 4, 4, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &PIQA&8, 8, 8, 8, 4, 12, 12, 12, 12, 10, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 10, 6, 4, 4, 4, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &Hella&8, 8, 8, 8, 2, 2, 4, 10, 10, 6, 10, 10, 10, 6, 6, 2, 2, 10, 2, 4, 2, 10, 10, 10, 4, 10, 10, 6, 6, 2, 8, 8\\
             \cmidrule{2-3}
             &Wino&8, 8, 8, 8, 8, 10, 4, 10, 4, 6, 6, 2, 10, 8, 12, 12, 10, 12, 12, 10, 6, 6, 8, 8, 10, 6, 6, 12, 2, 8, 8, 8\\
             \cmidrule{2-3}
             &ARC-e&8, 8, 8, 8, 4, 12, 12, 12, 12, 10, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 10, 6, 4, 4, 4, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &ARC-c&8, 8, 8, 8, 4, 12, 12, 12, 12, 10, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 10, 6, 4, 4, 4, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &OBQA&8, 8, 8, 8, 4, 12, 12, 12, 12, 10, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 10, 6, 4, 4, 4, 2, 12, 8, 8\\
            \cmidrule{1-3}
             \multirow{7}{*}{25\%} & BoolQ & 8, 8, 8, 8, 12, 2, 8, 2, 8, 12, 4, 2, 10, 12, 10, 4, 2, 2, 12, 8, 10, 2, 12, 12, 8, 4, 4, 2, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &PIQA&8, 8, 8, 8, 4, 2, 2, 10, 10, 2, 10, 10, 10, 2, 2, 2, 4, 10, 4, 6, 10, 2, 2, 6, 10, 2, 2, 10, 10, 2, 8, 8\\
             \cmidrule{2-3}
             &Hella&8, 8, 8, 8, 4, 10, 12, 12, 6, 10, 6, 6, 8, 2, 2, 12, 2, 12, 12, 6, 4, 10, 6, 2, 2, 8, 4, 2, 2, 8, 8, 8\\
             \cmidrule{2-3}
             &Wino&8, 8, 8, 8, 8, 4, 12, 8, 2, 2, 12, 2, 10, 12, 2, 12, 12, 10, 8, 12, 4, 6, 6, 4, 10, 4, 2, 10, 10, 12, 8, 8\\
             \cmidrule{2-3}
             &ARC-e&8, 8, 8, 8, 2, 12, 2, 6, 12, 6, 12, 10, 6, 4, 8, 8, 12, 2, 2, 6, 8, 4, 12, 12, 2, 4, 2, 6, 6, 2, 8, 8\\
             \cmidrule{2-3}
             &ARC-c&8, 8, 8, 8, 2, 12, 2, 6, 12, 6, 12, 10, 6, 4, 8, 8, 12, 2, 2, 6, 8, 4, 12, 12, 2, 4, 2, 6, 6, 2, 8, 8\\
             \cmidrule{2-3}
             &OBQA&8, 8, 8, 8, 4, 12, 12, 12, 12, 1, 8, 10, 6, 2, 8, 6, 8, 2, 8, 2, 8, 10, 12, 12, 10, 4, 4, 6, 2, 12, 8, 8\\
            \cmidrule{1-3}
              \multirow{7}{*}{30\%} & BoolQ & 8, 8, 8, 8, 12, 2, 8, 2, 8, 12, 4, 2, 10, 12, 10, 4, 2, 2, 12, 8, 10, 2, 12, 12, 8, 4, 4, 2, 2, 12, 8, 8\\
             \cmidrule{2-3}
             &PIQA&8, 8, 8, 8, 12, 6, 10, 4, 2, 4, 2, 4, 12, 8, 2, 2, 2, 12, 12, 12, 12, 2, 12, 4, 4, 2, 10, 2, 2, 8, 8, 8\\
             \cmidrule{2-3}
             &Hella&8, 8, 8, 8, 12, 6, 8, 4, 2, 12, 10, 4, 4, 2, 6, 4, 6, 10, 4, 2, 8, 6, 12, 10, 4, 6, 6, 6, 8, 2, 8, 8\\
             \cmidrule{2-3}
             &Wino&8, 8, 8, 8, 12, 6, 8, 4, 2, 12, 10, 4, 4, 2, 6, 4, 6, 10, 4, 2, 8, 6, 12, 10, 4, 6, 6, 6, 8, 2, 8, 8\\
             \cmidrule{2-3}
             &ARC-e&8, 8, 8, 8, 12, 6, 8, 4, 2, 12, 10, 4, 4, 2, 6, 4, 6, 10, 4, 2, 8, 6, 12, 10, 4, 6, 6, 6, 8, 2, 8, 8\\
             \cmidrule{2-3}
             &ARC-c&8, 8, 8, 8, 4, 10, 12, 12, 6, 10, 6, 6, 8, 2, 2, 12, 2, 12, 12, 6, 4, 10, 6, 2, 2, 8, 4, 2, 2, 8, 8, 8\\
             \cmidrule{2-3}
             &OBQA&8, 8, 8, 8, 12, 6, 8, 4, 2, 12, 10, 4, 4, 2, 6, 4, 6, 10, 4, 2, 8, 6, 12, 10, 4, 6, 6, 6, 8, 2, 8, 8\\
            \cmidrule{1-3}
             \multirow{7}{*}{50\%} & BoolQ & 8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &PIQA&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &Hella&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &Wino&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &ARC-e&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &ARC-c&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
             \cmidrule{2-3}
             &OBQA&8, 8, 8, 8, 12, 4, 6, 2, 2, 10, 4, 6, 12, 12, 2, 2, 12, 6, 4, 2, 6, 2, 4, 2, 6, 10, 10, 4, 2, 2, 8, 8\\
            \bottomrule
        \end{tabular}
    }\label{tab:con-llama13b}
\end{table*}

==> tabs/tab_main.tex <==
\begin{table*}[t]
    \centering
    \caption{Zero-shot performance of LLaMA-7B in unpruned, pruned, LoRA recovery, and RankAdaptor recovery. ‘Bold’ indicates the best performance at each pruning rate. Results are the optimal performance for each task. Specific $R$ configurations in Appendix \ref{app:r}. Reported in percentage (\%).}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{ll|ccccccc}
            \toprule
            Pruning Rate & Recover & BoolQ & PIQA & HellaSwag & WinoGrande & ARC-e & ARC-c & OBQA  \\
            \midrule
            {\parbox{1.8cm}{Rate = 0\%}} & - & 73.09 & 78.35 & 72.98 & 67.09 & 67.42 & 41.38 & 42.40  \\
            \cmidrule{1-9}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 20\%}} & w/o Tuning & 56.94 & 75.73 & 66.83 & 60.06 & 60.94 & 36.43 & 39.80 \\
            \cmidrule{2-9}
            & LoRA  & 63.30 & 76.82 & 68.68 & 63.38 & 63.76 & 37.11 & 40.60   \\
            \cmidrule{2-9}
            & RankAdaptor & \textbf{67.34} & \textbf{77.31} & \textbf{69.07} & \textbf{64.17} & \textbf{65.36} & \textbf{37.80} & \textbf{41.60}  \\
            \cmidrule{1-9}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 25\%}} & w/o Tuning & 59.94 & 73.23 & 62.35 & 58.80 & 55.81 & 34.90 & 39.40 \\
            \cmidrule{2-9}
            & LoRA  & 61.93 & 76.01 & 65.97 & 61.96 & 62.21 & 35.92 & 39.40  \\
            \cmidrule{2-9}
            & RankAdaptor & \textbf{67.43} & \textbf{76.06} & \textbf{66.08} & \textbf{64.40} & \textbf{62.63} & \textbf{36.77} & \textbf{40.40} \\
            \cmidrule{1-9}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 30\%}} & w/o Tuning & 58.96 & 71.22 & 58.10 & 58.88 & 52.19 & 32.34 & 38.40 \\
            \cmidrule{2-9}
            & LoRA  & 62.45 & 74.37 & 63.14 & 61.96 & 59.22 & 33.70 & 39.60  \\
            \cmidrule{2-9}
            & RankAdaptor & \textbf{66.21} & \textbf{75.19} & \textbf{63.61} & \textbf{63.14} & \textbf{60.10} & \textbf{34.64} & \textbf{40.20} \\
            \cmidrule{1-9}
            \multirow{5}{*}{\parbox{1.8cm}{Rate = 50\%}} & w/o Tuning & \textbf{57.98} & 60.94 & 34.35 & \textbf{52.25} & 31.82 & 27.30 & \textbf{35.80} \\
            \cmidrule{2-9}
            & LoRA  & 43.76 & 69.04 & 45.01 & 50.99 & 45.20 & \textbf{28.75} & 34.60   \\
            \cmidrule{2-9}
            & RankAdaptor & 51.65 & \textbf{69.48} & \textbf{45.03} & 51.93 & \textbf{45.66} & 28.41 & 35.00  \\
            \bottomrule
        \end{tabular}
    }\label{tab:res-llama7b}
\end{table*}

==> tabs/tab_mov.tex <==
\begin{table}
    \centering
    \begin{tabular}{c|c|c}
        \hline
        \text{Layer}  & \text{Fixed} & \text{Different} \\
        \hline
        1--8  & \multirow{4}{*}{8} & 4 \\
        9--16  &  & 6 \\
        17--24  &  & 10 \\
        25--32  &  & 12 \\
        \hline
    \end{tabular}
    \caption{Rank Value Configurations. Fixed refers to applying a constant rank value across multiple layers of the pruned model, while Different indicates assigning distinct rank values to different layers of the pruned model.}
    \label{tab:moti_config}
\end{table}

==> tabs/tab_res-llama13b.tex <==
\begin{table*}[ht]
    \centering
    \caption{Zero-shot performance of LLaMA-13B in unpruned, pruned, pruned with LoRA recovery, and pruned with RankAdaptor recovery settings; 'Bold' represents the best performance at the same pruning rate across the three pruned settings. The data in the table is from the optimal performance on each individual task. The results are reported in percentage (\%).}
    \resizebox{0.866\linewidth}{!}{
        \begin{tabular}{ll|ccccccc}
            \toprule
            Pruning Rate & Recover & BoolQ & PIQA & HellaSwag & WinoGrande & ARC-e & ARC-c & OBQA \\
            \midrule
            {\parbox{1.8cm}{Rate = 0\%}} & N/A & 68.50 & 79.11 & 76.21 & 70.09 & 74.58 & 44.54 & 42.20  \\
            \cmidrule{1-9}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 50\%}} & W/O Tuning & 58.90 & 66.32 & 42.24 & 52.25 & 39.06 & 29.18 & 33.20 \\
            \cmidrule{2-9}
            & LoRA  & 61.93 & 71.38 & \textbf{53.36} & 53.59 & 53.11 & 29.95 & 38.00  \\
            \cmidrule{2-9}
            & RankAdaptor & \textbf{62.05} & \textbf{71.71} & 53.33 & \textbf{54.22} & \textbf{53.20} & \textbf{30.89} & \textbf{39.40} \\
            \bottomrule
        \end{tabular}
    }\label{tab:res-llama13b}
\end{table*}

==> tabs/tab_res-llama7b-avg.tex <==
\begin{table*}[t]
    \centering
    \caption{Zero-shot performance of LLaMA-7B in unpruned, pruned, pruned with LoRA recovery, and pruned with RankAdaptor recovery settings; 'Bold' represents the best performance at the same pruning rate across the three pruned settings. The data in the table is from the overall performance across multiple tasks. The results are reported in percentage (\%).}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{ll|ccccccc|c}
            \toprule
            Pruning Rate & Recover & BoolQ & PIQA & HellaSwag & WinoGrande & ARC-e & ARC-c & OBQA & Average \\
            \midrule
            {\parbox{1.8cm}{Rate = 0\%}} & N/A & 73.09 & 78.35 & 72.98 & 67.09 & 67.42 & 41.38 & 42.40 & 63.10 \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 20\%}} & W/O Tuning & 56.94 & 75.73 & 66.83 & 60.06 & 60.94 & 36.43 & 39.80 & 56.96 \\
            \cmidrule{2-10}
            & LoRA  & 63.30 & 76.82 & 68.68 & 63.38 & 63.76 & 37.11 & 40.60 & 59.52  \\
            \cmidrule{2-10}
            & RankAdaptor & 66.91 & 76.93 & 68.78 & 63.14 & 65.24 & 37.54 & 40.80 & \textbf{59.90}  \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 25\%}} & W/O Tuning & 59.94 & 73.23 & 62.35 & 58.80 & 55.81 & 34.90 & 39.40 & 54.63 \\
            \cmidrule{2-10}
            & LoRA  & 61.93 & 76.01 & 65.97 & 61.96 & 62.21 & 35.92 & 39.40 & 57.63  \\
            \cmidrule{2-10}
            & RankAdaptor & 63.15 & 75.95 & 65.97 & 62.04 & 62.63 & 36.77 & 39.60 & \textbf{58.16} \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 30\%}} & W/O Tuning & 58.96 & 71.22 & 58.10 & 58.88 & 52.19 & 32.34 & 38.40 & 52.58 \\
            \cmidrule{2-10}
            & LoRA  & 62.45 & 74.37 & 63.14 & 61.96 & 59.22 & 33.70 & 39.60 & 56.63  \\
            \cmidrule{2-10}
            & RankAdaptor & 62.72 & 74.39 & 63.61 & 63.14 & 60.10 & 33.62 & 40.20 & \textbf{56.97} \\
            \cmidrule{1-10}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 50\%}} & W/O Tuning & 57.98 & 60.94 & 34.35 & 52.25 & 31.82 & 27.30 & 35.80 & 42.92 \\
            \cmidrule{2-10}
            & LoRA  & 43.76 & 69.04 & 45.01 & 50.99 & 45.20 & 28.75 & 34.60 & 45.62   \\
            \cmidrule{2-10}
            & RankAdaptor & 51.65 & 69.48 & 45.03 & 51.93 & 45.66 & 28.41 & 35.00 & \textbf{46.74}  \\
            \bottomrule
        \end{tabular}
    }\label{tab:res-llama7b-avg}
\end{table*}

==> tabs/tab_res-vicuna7b.tex <==
\begin{table*}[ht]
    \centering
    \caption{Zero-shot performance of Vicuna-7B in unpruned, pruned, pruned with LoRA recovery, and pruned with RankAdaptor recovery settings; 'Bold' represents the best performance at the same pruning rate across the three pruned settings. The data in the table is from the optimal performance on each individual task. The results are reported in percentage (\%).}
    \resizebox{0.866\linewidth}{!}{
        \begin{tabular}{ll|ccccccc}
            \toprule
            Pruning Rate & Recover & BoolQ & PIQA & HellaSwag & WinoGrande & ARC-e & ARC-c & OBQA  \\
            \midrule
            {\parbox{1.8cm}{Rate = 0\%}} & - & 75.69 & 77.75 & 71.06 & 67.80 & 69.07 & 40.78 & 42.20  \\
            \cmidrule{1-9}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 20\%}} & W/O Tuning & 52.35 & 76.17 & 64.79 & 59.59 & 65.99 & \textbf{38.14} & 40.00 \\
            \cmidrule{2-9}
            & LoRA  & 57.77 & \textbf{77.58} & 67.16 & 63.14 & 67.30 & 37.71 & 40.40   \\
            \cmidrule{2-9}
            & RankAdaptor & \textbf{61.19} & 77.15 & \textbf{67.32} & \textbf{63.85} & \textbf{67.68} & 38.05 & \textbf{41.20}  \\
            \cmidrule{1-9}
            \multirow{3}{*}{\parbox{1.8cm}{Rate = 25\%}} & W/O Tuning & 43.98 & 74.76 & 61.58 & 57.06 & 63.72 & \textbf{37.20} & 39.80 \\
            \cmidrule{2-9}
            & LoRA  & 50.34 & 75.24 & 64.10 & 61.33 & \textbf{63.93} & 35.67 & 40.60   \\
            \cmidrule{2-9}
            & RankAdaptor & \textbf{58.50} & \textbf{76.17} & \textbf{64.23} & \textbf{61.96} & 63.30 & 36.01 & \textbf{42.00}  \\
            \cmidrule{1-9}
             \multirow{3}{*}{\parbox{1.8cm}{Rate = 30\%}} & W/O Tuning & 43.12 & 73.45 & 55.64 & 57.22 & 58.96 & 34.30 & 37.80 \\
            \cmidrule{2-9}
            & LoRA  & \textbf{58.81} & 74.37 & 60.70 & \textbf{60.62} & 59.01 & 33.79 & 38.80   \\
            \cmidrule{2-9}
            & RankAdaptor & 57.58 & \textbf{75.57} & \textbf{61.63} & 60.22 & \textbf{60.94} & \textbf{34.81} & \textbf{39.00} \\
            \cmidrule{1-9}
             \multirow{3}{*}{\parbox{1.8cm}{Rate = 50\%}} & W/O Tuning & \textbf{62.29} & 60.28 & 33.91 & \textbf{54.54} & 35.14 & \textbf{28.16} & 33.80 \\
            \cmidrule{2-9}
            & LoRA  & 59.51 & 66.87 & 43.18 & 52.01 & 48.40 & 26.45 & 34.00  \\
            \cmidrule{2-9}
            & RankAdaptor & 59.91 & \textbf{67.46} & \textbf{43.50} & 52.41 & \textbf{48.70} & 27.65 & \textbf{35.80} \\
            \bottomrule
        \end{tabular}
    }\label{tab:res-vicuna7b}
\end{table*}
